Higher derivative terms including the Ramond-Ramond five-form

Superfield methods can be used to determine the precise way the self-dual five-form couples to the metric in the first non-trivial $\alpha'$ corrections to type IIB supergravity. We explicitly compute the exact tensor structure of these terms. This requires extensive use of computing algorithms to reduce the complicated expressions that appear to a surprisingly simple form. Along the way we show a new method of computing Schouten identities. With this result we clarify under which conditions one may neglect the five-form higher derivative terms. We comment on corrections to the thermodynamics of charged black holes.

==> Biblio.tex <==
\begin{thebibliography}{99}
%1
\bibitem{Maldacena} J. M. Maldacena, ``The large N limit of superconformal field theories and supergravity'',\\
\atmp{2}{1998}{231}, \hepth{9711200}.
%2
\bibitem{Tests} G. T. Horowitz, J. Polchinski, ``Gauge/gravity duality'', \grqc{0602037}.
%3
\bibitem{Magoo} O. Aharony, S. S. Gubser, J. Maldacena, H. Ooguri, Y. Oz, ``Large N field theories, string theory and gravity'', \prep{323}{2000}{183}
%4
\bibitem{Wald} R. M. Wald, ``Black hole entropy in the Noether charge'', \\ \prd{48}{1993}{3427}, \grqc{9307038}.
%5
\bibitem{Cloak} A. Dabholkar, R. Kallosh, A. Maloney, ``A Stringy cloak for a classical singularity'',\\ \jhep{12}{2004}{059}, \hepth{0410076}.
%6
\bibitem{SuperstarFull} K. Behrndt, A. H. Chamseddine, W. A. Sabra, ``BPS black holes in N=2 five dimensional AdS supergravity'',\\
\plb{442}{1998}{97}, \hepth 9807187.\\
K. Behrndt, M. Cvetic, W. A. Sabra, ``Non-extrene black holes of five dimensional N=2 AdS supergravity'',\\
\npb{553}{1999}{317}, \hepth{9810227}.
%7
\bibitem{Superstar} R. Myers, O. Tafjord, ``Superstars and giant gravitons'', 
\\\jhep{11}{2001}{009}, \hepth{0109127}.
%8
\bibitem{Invasion} J. McGreevy, L. Susskind, N. Toumbas, ``Invasion of the giant gravitons from Anti-de Sitter space'',\\
\jhep{06}{2000}{008}, \hepth{0003075}.
%9
\bibitem{LLM} H. Lin, O. Lunin, J. Maldacena, ``Bubbling AdS space and 1/2 BPS geometries'',\\ \jhep{10}{2004}{025}, \hepth{0409174}.
%10
\bibitem{Berenstein} D. Berenstein, ``A toy model for the AdS/CFT correspondence'',
\\ \jhep{07}{2004}{018}, \hepth{0403110}.
%11
\bibitem{Green} M. B. Green, C. Stahn, ``D3-branes on the Coulomb branch and instantons'',\\ \jhep{09}{2003}{052}, \hepth{0308061}.
%
%12
\bibitem{Superfield} M. B. Green, K. Peeters, C. Stahn, ``Superfield integrals in high dimensions'',\\ \jhep{08}{2005}{093}, \hepth{0506161}.
%
%13
\bibitem{Cadabra} K. Peeters, ``A field-theory motivated approach to symbolic computer algebra'', \\
{\it Comput. Phys. Commun.} {\bf 176} (2007) 550.
%14
\bibitem{Sugra} M. Gunaydin, G. Sierra and P.K. Townsend, ``Gauging the d=5 Maxwell-Einstein supergravity theories: more on Jordan algebras''\\ \npb{253}{1985}{573}.
%15
\bibitem{Lift} M. Cvetic, M.J. Duff, P. Hoxha, J.T.Liu. H. Lu, J.X. Lu, R. Martinez-Acosta, C.N. Pope, H. Sati, T.A. Tran, ``Embedding AdS black holes in ten-dimensions and eleven-dimensions'',\\
\npb{558}{1999}{96}, \hepth{9903214}.
%16
\bibitem{DualGiant} M. T. Grisaru, R. C. Myers, O. Tafjord, ``SUSY and Goliath'', \\ \jhep{08}{040}{2000}, \hepth{0008015}.
A. Hashimoto, S. Hirano, N. Itzhaki, ``Large branes in AdS and their field theory dual'',\\ \jhep{08}{2000}{051}, \hepth{0008016}.
%17
\bibitem{Witten} E. Witten, ``Anti-de Sitter space and holography'', \\
\atmp{2}{1998}{253}, \hepth{9802150}.
%18
\bibitem{Suranarayana} N. Suranarayana, ``Half-BPS giants, free fermions and microstates of superstars'',\\ \jhep{01}{2006}{082}, \hepth{0411145}.
%19
\bibitem{Mathur} S. D. Mathur, ``The fuzzball proposal for black holes: an elementary review'',\\
{\it Fortsch. Phys} {\bf 53} (2005) 793, \hepth{0502050}.
%20
\bibitem{Babel} V.Balasubramanian, J. de Boer, V. Jejjala, J. Simon, ``The Library of Babel: On the origin of gravitational thermodynamics'',\jhep{12}{2005}{006}, \hepth{0508023}.
%21
\bibitem{StretchedHor} L. D'Errico, W. Muck, R. Pettorino, ``Stretched horizon and entropy of superstars'',\\
 \jhep{05}{2007}{063}, \hepth{0703223}.
%22 
\bibitem{Sethi} M. B. Green, S. Sethi, ``Supersymmetry constraints on type IIB supergravity'',\\ \prd{59}{1999}{046006}, \hepth{9808061}.
%23
\bibitem{Gutowski} J. B. Gutowski, H. S. Reall, ``General supersymmetric AdS(5) black holes'',\\ \jhep{04}{2004}{048}, \hepth{0401129}.
%24
\bibitem{SugraIIB} J. H. Schwarz, ``Covariant field equations of chiral N = 2 D = 10 supergravity'',\\
\npb{226}{1983}{269}.
%25
\bibitem{Fulling} S. A. Fulling, R. C. King, B. G. Wybourne, and C. J. Cummins, ``Normal forms for
tensor polynomials. 1: The Riemann tensor'',\\
\cqg{9}{1992}{1151}.
%26
\bibitem{xTensor} J. Martin-Garcia, ``xPerm and xAct'',\\
http://metric.iem.csic.es/Martin-Garcia/xAct/index.html.
%27
\bibitem{Mathematica} Wolfram Research, Inc., Mathematica, Version 5.0, Champaign, IL (2003).
%28
\bibitem{Portugal} R. Portugal, ``Algorithmic simplification of tensor expressions'', {\it J. Phys} {\bf A32} (1999) 7779.
%29
\bibitem{LeadingOrder} K. Peeters, A. Westerberg, ``The Ramond-Ramond sector of string theory beyond leading order'',\\
\cqg{21}{2004}{1643}, \hepth{0307298}.
\end{thebibliography}



